LARGE: Latent-Based Regression through GAN Semantics

We propose a novel method for solving regression tasks using few-shot or weak supervision. At the core of our method is the fundamental observation that GANs are incredibly successful at encoding semantic information within their latent space, even in a completely unsupervised setting. For modern generative frameworks, this semantic encoding manifests as smooth, linear directions which affect image attributes in a disentangled manner. These directions have been widely used in GAN-based image editing. We show that such directions are not only linear, but that the magnitude of change induced on the respective attribute is approximately linear with respect to the distance traveled along them. By leveraging this observation, our method turns a pre-trained GAN into a regression model, using as few as two labeled samples. This enables solving regression tasks on datasets and attributes which are difficult to produce quality supervision for. Additionally, we show that the same latent-distances can be used to sort collections of images by the strength of given attributes, even in the absence of explicit supervision. Extensive experimental evaluations demonstrate that our method can be applied across a wide range of domains, leverage multiple latent direction discovery frameworks, and achieve state-of-the-art results in few-shot and low-supervision settings, even when compared to methods designed to tackle a single task.

==> figures/cat_sort_first_afhq.tex <==
\begin{figure}[!hbt]
\setlength{\tabcolsep}{1pt}
    \centering
    \begin{tabular}{c c}
        \raisebox{0.04\textwidth}{Yaw} & \includegraphics[width=\linewidth]{images/cat_sort/all_sorted_factor_6_2_start_idx_0.png} \\
        \raisebox{0.04\textwidth}{Age} & \includegraphics[width=\linewidth]{images/cat_sort/all_sorted_factor_1_2_start_idx_0.png} \\
        \raisebox{0.04\textwidth}{Pitch} & \includegraphics[width=\linewidth]{images/cat_sort/all_sorted_factor_8_7_start_idx_0.png} \\
    \end{tabular}
    \caption{}
    \label{fig:sort_10_first_afhq_cats}
\end{figure}

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}

==> paper_summary.tex <==
\section{Temp paper summary}

\paragraph{Improve ImageNet with GANs}

\cite{ravuri2019seeing} Demonstrates that although BigGAN generates good looking images, training a classifier on its output leads to a big drop in performance as compared to training on real images from ImageNet. Combining the two datasets leads to a minor boost in performance.

\cite{shmelkov2018good} "show that all popular GANs consistently under-perform by a significant margin against classifiers trained on real images".

\cite{ravuri2019classification} This is a different version of \cite{ravuri2019seeing}

\cite{besnier2020dataset} Propose three separate methods to boost performance of training on BigGAN images which are - Hard Sample Mining, Dataset Smoothing (replacing the dataset gradually) and Batch Norm statistics Adaptation.

\cite{wang2018low} proposes a meta-learning method that learns to generate new samples which are beneficial for training of a classifier. They optimize through from the classifier through the image and until the generator, so the generator generates the images the help the classifier most. They don't use a discriminator, the generated images might not be realistic.

\cite{perez2017effectiveness} discusses the effectiveness of number of methods for augmentations. They compare naive augmentation with some more complex ones. They experiment with cycleGAN trained for style-transfer. They find that GANs are usually not superior to basic augmentation but are much more expensive. They propose an additional neural network (similar to \cite{wang2018low}, but no-meta learning, just end-to-end augmentations) that learns to augment a given image and then both the augmented and natural image are used as inputs for classification. 

\cite{antoniou2017data} Proposes a meta-learning method that takes data from a source domain and generalise it to generate other within-class data items. This method does not depend on the classes, thus can be applied to unseen classes. They showed great improvement in low data regime classification tasks.

\paragraph{Semi-Supervised}

\cite{springenberg2015unsupervised} The D in GANs can be used as an unsupervised classifier according to some prior on the data. In semi-supervised setting, the above could be one loss and another loss is a simple CE.

\cite{odena2016semi, salimans2016improved} propose a similar approach for semi-supervised setting. The dataset has K classes and the classifier is tasked to output either one of the K classes or "FAKE". Then the classifier is trained both on the real data and also as a discriminator against a generator. 

\paragraph{Motivation for using DGM for classification training}

Most papers mentioned here consider DGM as method for data augmentation in the sense that they generate more data. \cite{ratner2017learning} use GAN to learn augmentations for existing images.
\cite{marriott2020assessment} demonstrates anonymization of face datasets. They train GANs on faces and demonstrate that the generated identities are different than those in the training data. 

\paragraph{Using Latent space editing}

\cite{ramaswamy2020fair} uses latent space editing in PGGAN to augment an existing dataset (CelebA) to solve biases. Suppose there are two correlated properties in the dataset: to wear sunglasses and a hat. The generator trained on such dataset will usually generate images with both or neither. They learn SVM in latent space for the two properties using pretrained classifiers (similar to InterFaceGAN). Then, given a vector z they create an edited version of it- z' which decorrelate the attributes, by being positive for one and negative for the other. They train a classifier on the original dataset & images generated from z and z'. The accuracy precision improves as well as some fairness metrics.

\cite{denton2019detecting} also concerns bias and fairness but is much different. It performs linear edits in latent space of PGGAN and test how much a pretrained smile classifier changes with respect to attributes like "Young", "Beard".

\cite{viazovetskyi2020stylegan2} uses latent space editing in StyleGAN to generate pairs of images. One image is the semantic edit of another. Then they train a pix2pixHD network between these pairs. We can learn how to collect paired data from them.

\paragraph{Data-free knowledge transfer}

\cite{yin2020dreaming} propose a method to invert a pretrained classifier, without access to data. This allows to generate class-conditional images that should be similar to the training data. They demonstrate a few applications for this ability, one of them being knowledge-transfer. They take a pretrained Resnet50v1.5 imagenet classifier with TOP-1 acc 77.26\%, and invert it to generate 140K new images. Then a new classifier with the same architecture is trained from scratch, and achieves TOP-1 acc of 73.8\%.

\paragraph{Other}

\cite{frid2018gan} "generated synthetic samples of three classes of liver lesions individually, using three DCGANs
to improve the task of lesion classification".

\cite{zhu2017data} use simple CycleGAN to generate more data for minority classes for facial expression classification. Improved results.

\cite{sixt2018rendergan} use a GAN to generate more data for bee identification. The GAN generates an image and parameters for a fixed set of augmentations (blur, lighthing, etc.) to be applied on that image  

\cite{mun2017generative} the wierd paper with the DB and SVM.

==> tables/ablation_inversion.tex <==
\begin{table}[!hbt]
    \centering
    \caption{Pose estimation accuracy as a function of the number of training samples viewed when conducting inversions using three off-the-shelf encoders.}
    \begin{tabular}{c|c|c|c}
        \# calibration samples & pSp & e4e & ReStyle \\ \hline
        2 & $4.55 \pm 1.72$ & $4.30 \pm 1.20$ & $4.89 \pm 1.88$ \\ 
        5 & $3.80 \pm 0.86$ & $3.59 \pm 0.58$ & $4.07 \pm 1.05$ \\ 
        10 & $3.52 \pm 0.64$ & $3.30 \pm 0.30$ & $3.75 \pm 0.64$ \\ 
        20 & $3.34 \pm 0.32$ & $3.16 \pm 0.19$ & $3.52 \pm 0.31$ \\ 
        1000 & $3.09 \pm 0.00$ & $2.97 \pm 0.00$ & $3.28 \pm 00$
    \end{tabular}

    \vspace{-5pt}
    \label{tbl:ablation_inversion}
\end{table}

==> tables/ablation_mapping.tex <==
\begin{table}[!hbt]
    \centering
    \begin{tabular}{c|c|c|c}
        \# calibration samples & Best Layer & Weighted Distance & All layers \\ \hline
        2 & - & - & - \\ 
        5 & - & - & - \\ 
        10 & - & - & - \\ 
        20 & - & - & - \\
        1000 & - & - & -
    \end{tabular}
    \caption{Layer weighting results. In each row, we show the MAE of predictions obtained when using a \w boundary and projecting it to all channels of \wplus . We demonstrate results when considering only the best layer, our weighted-layer distance, or considering all layer distances as a set of 18 features. Our weighted distance obtains the best results at low supervision, and comparable results at high supervision setups.}
    \vspace{-5pt}
    \label{tbl:ablation_mapping}
\end{table}

==> tables/numeric_regression.tex <==
\setlength\tabcolsep{3pt}
\begin{table}[]
    \centering
    \caption{Caption}
    
    \begin{tabular}{|c c | c c c c c}
        \hline
         \multirow{2}{*}{Dataset} & \multirow{2}{*}{Property} & \multicolumn{5}{c|}{number of labeled samples} \\ \multicolumn{2}{c|}{} & 2 & 5 & 10 & 20 & 1000  \\
         \hline
        %  \multirow{2}{*}{Faces} & \texttt{A} & \textbf{0.03} & \textbf{0.17} & \textbf{25.17} & 48.72 & \textbf{62.46} & 48.75 \\
        %  & \texttt{D} & 0.05 & 0.23 & 30.96 & \textbf{40.54} & 81.08 & \textbf{43.63} \\
        %  \hline
        %  \multirow{2}{*}{Cars} & \texttt{A} & 0.10 & 0.32 & \textbf{10.56} & \textbf{22.08} & \textbf{12.92} & \textbf{24.30} \\
        %  & \texttt{D} & 0.10 & 0.32 & 12.18 & 22.71 & 15.44 & 26.83 \\
        % \hline
        %  \multirow{2}{*}{Horse} & \texttt{A} & \textbf{0.11} & \textbf{0.36} & \textbf{34.13} & 35.79 & 40.48 & \textbf{31.84} \\
        %  & \texttt{D} & 0.16 & 0.45 & 37.07 & \textbf{31.91} & \textbf{35.31} & 32.18 \\
        % \hline
        %  \multirow{2}{*}{Cats} & \texttt{A} & \textbf{0.10} & \textbf{0.41} & \textbf{42.60} & \textbf{32.83} & \textbf{217.44} & \textbf{45.13} \\
        %  & \texttt{D} & 0.14 & 0.48 & 49.90 & 40.59 &  222.30 & 51.07 \\
        % \hline
        %  \multirow{2}{*}{Church} & \texttt{A} &  \textbf{0.09} &  \textbf{0.32} &  \textbf{25.96} & 38.90 & 26.91 & 29.63 \\
        %  & \texttt{D} & 0.13 & 0.40 & 27.09 &  \textbf{31.18} & \textbf{21.87} & \textbf{23.32} \\
        % \hline
    \end{tabular}
    \label{tab:tradeoff-results}
\end{table}

